From approximation error to optimality gap -- Explaining the performance impact of opportunity cost approximation in integrated demand management and vehicle routing

The widespread adoption of digital distribution channels both enables and forces more and more logistical service providers to manage booking processes actively to maintain competitiveness. As a result, their operational planning is no longer limited to solving vehicle routing problems. Instead, demand management decisions and vehicle routing decisions are optimized integratively with the aim of maximizing revenue and minimizing fulfillment cost. The resulting integrated demand management and vehicle routing problems (i-DMVRPs) can be formulated as Markov decision process models and, theoretically, can be solved via the well-known Bellman equation. Unfortunately, the Bellman equation is intractable for realistic-sized instances. Thus, in the literature, i-DMVRPs are often addressed via decomposition-based solution approaches involving an opportunity cost approximation as a key component. Despite its importance, to the best of our knowledge, there is neither a technique to systematically analyze how the accuracy of the opportunity cost approximation translates into overall solution quality nor are there general guidelines on when to apply which class of approximation approach. In this work, we address this research gap by proposing an explainability technique that quantifies and visualizes the magnitude of approximation errors, their immediate impact, and their relevance in specific regions of the state space. Exploiting reward decomposition, it further yields a characterization of different types of approximation errors. Applying the technique to a generic i-DMVRP in a full-factorial computational study and comparing the results with observations in existing literature, we show that the technique contributes to better explaining algorithmic performance and provides guidance for the algorithm selection and development process.

==> abstract.tex <==
The widespread adoption of digital distribution channels both enables and forces more and more logistical service providers to manage booking processes actively to maintain competitiveness. As a result, their operational planning is no longer limited to solving vehicle routing problems. Instead, demand management decisions and vehicle routing decisions are optimized integratively with the aim of maximizing revenue and minimizing fulfillment cost. The resulting integrated demand management and vehicle routing problems (i-DMVRPs) can be formulated as Markov decision process models and, theoretically, can be solved via the well-known Bellman equation. Unfortunately, the Bellman equation is intractable for realistic-sized instances. Thus, in the literature, i-DMVRPs are often addressed via decomposition-based solution approaches involving an opportunity cost approximation as a key component. Despite its importance, to the best of our knowledge, there is neither a technique to systematically analyze how the accuracy of the opportunity cost approximation translates into overall solution quality nor are there general guidelines on when to apply which class of approximation approach. In this work, we address this research gap by proposing an explainability technique that quantifies and visualizes the magnitude of approximation errors, their immediate impact, and their relevance in specific regions of the state space. Exploiting reward decomposition, it further yields a characterization of different types of approximation errors. Applying the technique to a generic i-DMVRP in a full-factorial computational study and comparing the results with observations in existing literature, we show that the technique contributes to better explaining algorithmic performance and provides guidance for the algorithm selection and development process. \\[0.1cm]

==> notation.tex <==
\section{Notation}\label{app: notation}
\begin{align*}
	&t = 1,..., T && \text{decision epoch}\\
	&s_t && \text{state in period } t\\
	&s_{tc} && \text{state element indicating the number of customer orders of type } c\\
	&c \in \mathcal{C} = \{1,...,C\} && \text{customer order type}\\
	&\lambda_{c}(t) && \text{arrival probability of a customer request from customer order type } c \text{ in decision epoch } t\\
	&\lambda_0(t) && \text{probability that no customer request arrives in decision epoch } t\\
	&c_t && \text{customer requesting in period } t\\
	&e_{c_t} && \text{unit vector with entry 1 for the customer order type } c \text{ the current customer request } c_t {\text belongs to}\\
	&l_c && \text{location of customer order type } c\\
	&r_c && \text{revenue of customer order type } c\\
	&\mathcal{R} && \text{set of customer order revenues}\\
	&\mathcal{L} && \text{set of delivery locations}\\
	&\tilde{\mathcal{L}}_t && \parbox[t]{.6\textwidth}{\text{set of nodes for locations of which one or more customer requests already turned } \text{into confirmed customer order before decision epoch} t}\\
	&\ell(l_c) && \text{node for location } l_c\\
	%&s_{ki} \in \{0, 1\} && \text{element of statevector, } 1 \text{, if customer request } i \text{ is accepted before periode } k, 0 \text{, otherwise}\\
	& \mathcal{N}_{t} && \text{set of customer requests that are accepted before period } t\\
	&a_t \in \{0, 1\} && \text{action in period } t, 0 \text{, if customer request arriving in } t \text{ is rejected, } 1 \text{, otherwise}\\
	%&r_{c_i} && \text{reward per order } c_i\\
	&V_t(s_t) && \text{value of state } s_t\\
	&\mathbb{E}(R(\mathcal{N}^+_{t}) \mid s_t) && \text{expected future revenues given state } s_t\\
	&\mathbb{E} (C(s_{T+1})\mid s_t) && \text{expected future routing costs given state } s_t\\
	&\Delta V_t(s_t,c_t) && \text{opportunity cost of customer request } c_t \text{ in state } s_t\\
	&\Delta V_t(s_t,c_t) && \text{opportunity cost of customer request } c_t \text{ in state } s_t\\
	&\Delta \mathbb{E}(R(\mathcal{N}^+_{t}) \mid s_t, c_t) && \text{DPC of customer request } c_t \text{ in state } s_t\\
	&\Delta \mathbb{E} (C(s_{T+1})\mid s_t, c_t) && \text{MCTS of customer request } c_t \text{ in state } s_t\\
	&\pi && \text{policy}\\
	&\pi^t && \text{period-dependent policy}\\
	&V^{\pi}(s_t) && \text{value of state } s_t \text{ when following policy } \pi\\
	&s_{t+1} \mid s_t, a_t && \text{successor state if in state } s_t\text{ action } a_t \text{ is taken}\\
	&\Gamma(s_t) && \text{subtree/decision tree that is the child of node } s_t\\
	&V(\Gamma(s_t)) && \text{value of subtree/decision tree } \Gamma(s_t)\\
%	&\mathcal{A} && \text{set of accepted customer requests}\
	&\mathcal{N}^+_{t} && \parbox[t]{.6\textwidth}{\text{set of customer requests that are being accepted after period } t \text{ until the end of the booking period} T}\\
	& \mathcal{S}(\cdot) && \text{space of feasible solutions of a problem }\\
	& VRP_\tilde{\mathcal{L}} && \text{vehicle routing problem solved over nodes } \tilde{\mathcal{L}}\\
	& C(s_{T+1}) && \text{routing costs in a final state } s_{T+1}
\end{align*}

